Does Robustness Improve Fairness? Approaching Fairness with Word Substitution Robustness Methods for Text Classification

Existing bias mitigation methods to reduce disparities in model outcomes across cohorts have focused on data augmentation, debiasing model embeddings, or adding fairness-based optimization objectives during training. Separately, certified word substitution robustness methods have been developed to decrease the impact of spurious features and synonym substitutions on model predictions. While their end goals are different, they both aim to encourage models to make the same prediction for certain changes in the input. In this paper, we investigate the utility of certified word substitution robustness methods to improve equality of odds and equality of opportunity on multiple text classification tasks. We observe that certified robustness methods improve fairness, and using both robustness and bias mitigation methods in training results in an improvement in both fronts

==> archive.tex <==

\subsection{Augmenting Datasets to create Fairness and Robustness Models}
To measure robustness, we follow Jia et al's approach of, given a dataset B, creating an adversarial test set $B_{pb}$ that has been augmented with label-preserving word substitutions using word substitutions that does not decrease the log-likelihood of the text under a pre-trained language model by more than some threshold. More details for each of the various datasets are below. We denote these adversarial test sets as $TrustPilot_{p}$, $TC_{p}$, and $BiasinBios_{pb}$. 

Additionally, in order to evaluate the notion of Counterfactual Fairness, we construct a fairness test set $B_{pb}$, which consists of perturbations of gender words, as well as second-order indirect bias. Previous work [Gonen et al, Bolukbasi et al] has shown that even when direct bias is removed, indirect bias still exists in words that are associated with particular protected groups (for example, associating football with DJ, and softball with receptionist). We thus construct a set of indirect bias as well as direct bias perturbations for our fairness CFA set. We do so via a two staged approach: 
1. We first find a set of the most biased words, where the bias of a word $w$ is defined as $cos(w, g)$ where g is the gender subspace. For these sets of experiments, we find the 1,000 most biased words.
2. For each word in each sentence, we find the newest words. 
 
Following Alzantot et al \cite{https://arxiv.org/abs/1804.07998}, we use a language model to gauge for the appropriateness of word substitutions - for example, "he had a baby" does not make sense. For gendered words, we take into account gendered names as well as pronouns and nouns. We use the method by Alzantot et al, using the counter-fitted word vectors from Mrksic et al, to find the space of gendered names and pronouns that preserve semantic meaning. 


Several strands of debiasing have emerged: adversarial approaches and post processing debiasing of word and contextualized sentence embeddings. 


-----------------
Previous

As natural language processing systems are increasingly used in our daily lives, it is important that the models used are robust and fair to ensure that unintended outcomes for end users are minimized, and that  models do not offer disparate experiences to customers from diverse backgrounds. In NLP, robustness to word substitutions is widely studied, which ensures that machine learning systems are able to handle inputs that differ spuriously from the datasets they were trained in. This is common in real world textual settings since there are multiple ways to communicate similar concepts.

Prior work has optimized for each of these objectives, and yet to our knowledge, there are no studies on the effect of optimizing for word substitution robustness on fairness, or that of optimizing fairness for word substitution robustness. Our main contribution is to be the first study to do so.  

A natural question is to why it would make sense to expect a model optimized for word substitution robustness to improve fairness, or vice versa. The aim of robustness methods is to ensure that models are robust against any spurious changes to an example that should not change the ground truth label associated with it. This corresponds to notions of fairness such as counterfactual fairness, since gold labels should not be dependent on gender information present in an example in most non-gender related tasks.  On the other hand, fairness methods have been shown to also reduce spurious associations between words not directly related to sensitive attributes, or indirect bias \citep{Bolukbasi2016ManIT}, which may help with word substitution robustness. 

We focus on text classification tasks, as many important industry applications such as domain and intent classification falls under text classification \cite{Su2018ARS}. 
We explore the relationship between robustness and fairness with GloVe-based CNN models \citep{Kim2014ConvolutionalNN} and Interval Bound Propagation (IBP) \citep{Jia2019CertifiedRT}, and BERT \citep{bert} with SAFER \citep{Ye2020SAFERAS}, and focus on popular fairness methods.

We find that while fairness methods slightly improve robustness, robustness methods achieve not only robustness, but also fairness to almost the same level as fairness methods. Furthermore, combining both fairness and robustness shows improvement in both fronts, and in some cases exceeded performance from training on only fairness or robustness alone. We also conduct model interpretability studies to understand the decision making of models once trained using robustness and fairness methods. We make observations such as robustness methods decreases feature importance to sensitive gender tokens 

\begin{table}[]
\begin{tabular}{|p{3cm}|p{3cm}|}
\hline
\textbf{Model} & \textbf{Gender tokens present in the list of features that appear in the top 5 features in the set of examples that the baseline got wrong and IBP model got correct} \\ \hline
Baseline model & He, she, man, men, guy, her, him \\ \hline
Baseline model + IBP & he, her, him \\ \hline
\end{tabular}
\caption{\label{font-table} Most common tokens from LIME experiments}
\end{table}

\begin{figure*}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/LIME_jigsaw.png}
    \caption{Frequency of gender token features as extracted by LIME for baseline and IBP trained models. We see a decrease in number and frequency of gender tokens in the list of top-5 most important features.}
    \label{fig:atzeni_trad}
  \end{subfigure}
  \hfill 
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth, height=3.25cm]{images/all_tokens.png}
    \caption{Frequency of gender token features as extracted by LIME for baseline and SAFER trained models. We see a decrease in number and frequency of gender tokens in the list of top-5 most important features..}
    \label{fig:atzeni_sls}
  \end{subfigure}
  \caption[.]{LIME results on Jigsaw Toxicity}
  \label{fig:lamp}
\end{figure*}


\begin{figure*}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/orig_saliency1.png}
    \caption{Baseline}
    \label{fig:atzeni_trad}
  \end{subfigure}
  \hfill 
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/ibp_saliency1}
    \caption{IBP}
    \label{fig:atzeni_sls}
  \end{subfigure}
  \caption{Gradient saliency map (example 1)}
  \label{fig:lamp}
\end{figure*}
\begin{figure*}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{images/orig_saliency2.png}
    \caption{Baseline}
    \label{fig:atzeni_trad}
  \end{subfigure}
  \hfill 
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth,]{images/ibp_saliency2}
    \caption{IBP}
    \label{fig:atzeni_sls}
  \end{subfigure}
  \caption[.]{Gradient saliency map (example 2)}
  \label{fig:lamp}
\end{figure*}


PREVIOUS IBP_JIGSAW 
\begin{table*}[h!]
\centering
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}| p{1.5cm}|p{1.5cm}| p{2cm}| }
\hline \textbf{Model} &  \textbf{FPED} & \textbf{FNED} & \textbf{TPED} & \textbf{Certified Robustness Metric (Lower Bound)} & \textbf{Raw task AUC} & \textbf{FairOverall}\\ \hline
Baseline (CNN) & 0.907 & 1.91 & 0.311 & 0.27 & 0.957 & 3.128 \\ %0.87 
\hline
GloVe + CNN +  IBP &  \textbf{0.0} &  \textbf{0.033} & \textbf{0.179} & \textbf{0.934} & \textbf{0.913} & 1.146 \\
\hline 
GloVe + CNN +  IBP_{gender} & \textbf{0.009} & \textbf{0.014} & \textbf{0.175} & \textbf{0.912} & \textbf{0.947}& 1.101 \\
\hline
GloVe + CNN +  Instance weighting &  \textbf{0.25} & 2.05 & 0.309 & \textbf{0.214} & 0.955  & 2.609 \\
\hline
GloVe + CNN +  IBP + Instance weighting&  \textbf{0.02} & \textbf{0.19} & \textbf{0.163} & \textbf{0.942} & \textbf{0.889}&  0.373 \\
\hline
GloVe + CNN +  $HardDebias$  & \textbf{0.339} &  \textbf{0.17} & \textbf{0.144} & \textbf{0.404} & 0.951 & 0.65 \\
\hline
GloVe + CNN +  IBP + $HardDebias$  &  \textbf{0.23} & \textbf{0.15} & \textbf{0.24} & \textbf{0.89} & \textbf{0.923} & 0.62 \\
%\hline
%GloVe + CNN +  Adversarial Training (Demographic Parity) &  1.81 & 1.23  & 0.303 & 0.534 & 0.89 \\
\hline
GloVe + CNN +  Adversarial Training (Equalized Odds) & \textbf{1.898} & \textbf{2.26}  &  \textbf{0.1877} & \textbf{0.644} & 0.955 & 4.35 \\
\hline
GloVe + CNN +  IBP + Adversarial Training (Equalized Odds) & \textbf{0.068} & \textbf{0.061} &  0.29 & \textbf{0.901}   & \textbf{0.92} & 0.419 \\

\hline
\end{tabular}
\caption{\label{font-table} Experiment results on CNN baseline model for Jigsaw dataset. The bolded numbers represent numbers that are statistically significant in difference with the baseline number (p $<$ 0.05). We can see that adding IBP improves fairness. }
\label{table:jigsawresults}
\end{table*}



BIB IBP:

\begin{table*}[h!]
\centering
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}| p{2cm}|p{1.5cm}| }
\hline \textbf{Model} &  \textbf{FPED} & \textbf{FNED} & \textbf{$TPR_{diff}$} & \textbf{Certified Robustness Metric (Lower Bound)} & \textbf{Raw task accuracy}\\ \hline
GloVe + CNN & 0.1275 & 0.1368 & 0.131 & 0.115 & 0.787 \\
\hline
GloVe + CNN + IBP & 0.1244 & 0.1325 & 0.127 & \textbf{0.702} & \textbf{0.743} \\
\hline 
GloVe + CNN + IBP_{gender} & 0.1197 & \textbf{0.1273}   & \textbf{0.104} & \textbf{0.711} & \textbf{0.749}  \\
\hline
GloVe + CNN + Instance weighting & 0.1061 & \textbf{0.1132}  & \textbf{0.118} & \textbf{0.095} & \textbf{0.755}  \\
\hline
GloVe + CNN + Instance weighting + IBP& \textbf{0.1093} & 0.1104 & \textbf{0.113}  & \textbf{0.719} & \textbf{0.732}  \\
\hline 
GloVe $HardDebias$ + CNN  &  0.1184 & 0.1241 & \textbf{0.106} & \textbf{0.07} & 0.767 \\
\hline
 $HardDebias$ + CNN + IBP &  \textbf{0.115} & \textbf{0.1282} & \textbf{0.101} & \textbf{0.715} & \textbf{0.735} \\
\hline
Adversarial Training + CNN  &  0.1167 & 0.1220 & \textbf{0.114} & \textbf{0.18} & 0.773 \\
\hline
 Adversarial Training + CNN + IBP &  \textbf{0.1138} & \textbf{0.1268} & \textbf{0.112} & \textbf{0.693} & \textbf{0.725} \\
\hline
\end{tabular}
\caption{\label{font-table} Experiment results on CNN baseline model for Bias in Bios dataset}
\label{table:ibpresults}
\end{table*}


Jigsaw + SAFER 
\begin{table*}[]
\centering
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}| p{1.5cm}|p{1.5cm}| p{2cm}|}
\hline \textbf{Model} &  \textbf{FPED} & \textbf{FNED} & \textbf{TPED} & \textbf{Certified Robustness Metric (Lower Bound)} & \textbf{Raw task accuracy} & \textbf{FairOverall}\\ \hline
BERT & 0.29 & 0.138 & 0.263 & 0.95 & 0.914 & 0.691\\
\hline
BERT + SAFER & 0.29 & 0.104  &0.142 & 0.967 & 0.918 & 0.536 \\
\hline
BERT + SAFER_{gender} & 0.286 & 0.117 & 0.171 &  0.968 & 0.917 & 0.574 \\
\hline
\end{tabular}
\caption{\label{font-table} Model performance on BERT and SAFER for Jigsaw dataset}
\end{table*}

BIB + SAFER
\begin{table*}[]
\centering
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}| p{1.5cm}|p{1.5cm}| p{2cm}|}
\hline \textbf{Model} &  \textbf{FPED} & \textbf{FNED} & \textbf{$TPR_{diff}$} & \textbf{Certified Robustness Metric (Lower Bound)} & \textbf{Raw task accuracy} & \textbf{FairOverall}\\ \hline
BERT & 0.1317 & 0.145 & 0.148 & 0.164 & 0.796 & 0.425 \\
\hline
BERT + SAFER & 0.1147 & 0.1285  & 0.134 & 0.726 & 0.744 & 0.377 \\
\hline
BERT + SAFER_{gender} & \textbf{0.1129} & 0.1261  & \textbf{0.097} & 0.733 & 0.761 & 0.336\\
\hline
\end{tabular}
\caption{\label{font-table} Model performance on BERT and SAFER for Bias in Bios dataset}
\end{table*}

%\begin{itemize}
 Instance weighting \citep{Zhang2020DemographicsSN} is a method to debias text classification models for bias against examples containing identity-terms (for example, "gay" or ``black") by weighting the instances in the loss function to account for presence of such bias in the training dataset. Given example $x$ and label $y$, and group identity term $z$ present in $x$, Zhang et al proposed to use the weight \textit{w} = $\frac{Q(y)}{P(y|z)}$ for instance \textit{((x,z), y)} in the loss function. Instance weighting optimizes for demographic parity \citep{Zafar2017FairnessCM}, which is the notion that decisions should not be based on protected attributes. Formally, a model fulfills demographic parity if in its predictions, the outcomes \textit{X} and protected attributes \textit{Y} are independent from each other.

$HardDebias$ and $SoftDebias$ \citep{Bolukbasi2016ManIT} are methods to 
reduce representational harm existent in word embeddings that has demonstrated improvement in downstream fairness. Inspired by this work, we use hard debiased embeddings to initialize our CNN-based models.

Adversarial debiasing \citep{Zhang2018MitigatingUB} is a method that uses adversarial training to achieve fairness. 
Consider a model with weights W that minimizes loss $L_p(\bar{y}, y)$ and an adversary, or discriminator, with weights U that tries to predict the protected attribute $z$ from model predictions $\bar{y}$ and ground truth \textit{y} by minimizing loss $L_A(\bar{z}, z)$, Zhang et al. proposes to use adversarial style training to create a debiased model. The model weights W are updated via the below equation to encourage the model to try to hurt adversarial performance: 
$ \triangledown_W L_P - proj_{\triangledown_{W}L_{A}} \triangledown_{W}L_{P} - \alpha \triangledown_{W}L_{A}$. Adversarial debiasing can be used to optimize for either equality of opportunity, equality of odds, or demographic parity. 

RobustnEss FaIrNEss (REFINE)


\begin{table*}[h!]
\small
\centering
\begin{tabular}{p{4.5cm}p{2cm}p{1.5cm}p{1.5cm}p{1.5cm}p{2cm}}
\toprule 
\multirow{2}{*}{Model} & {Raw task} & \multicolumn{3}{c}{{Fairness}} & {Robustness}  \\
\cmidrule(lr){2-2}\cmidrule(lr){3-5} \cmidrule(lr){6-6}
  &  {AUC}&  {EOdds} & {FPED} & {TPED} & {CRA} \\ 
  \midrule
Baseline & 0.957 & 1.218 & 0.907  & 0.311  & 0.270   \\ %0.87 
\midrule
 IBP &  0.913 & 0.179 & 0.0 &  \textbf{0.179}  & \textbf{0.934}   \\
 $\text{IBP}_\text{gender}$ &  \textbf{0.947} &  0.184 &  \textbf{0.009} & \textbf{0.175}   & \textbf{0.912} \\
  \midrule
 Instance weighting &  0.955 & 0.559  & \textbf{0.25}  & 0.309 & \textbf{0.214}   \\
  \textit{HardDebias}  & 0.951 &  0.509 & \textbf{0.339} &  \textbf{0.144}   & \textbf{0.404}  \\
   Adversarial Training& 0.955 & 2.086 &  \textbf{1.898}  &  \textbf{0.188}  &  \textbf{0.644}   \\
  \midrule
 IBP + Instance weighting& \textbf{0.889} & 0.165 & \textbf{0.02}  & \textbf{0.163}  & \textbf{0.942}  \\
IBP + \textit{HardDebias}   & \textbf{0.923} &  0.47 & \textbf{0.24} &  \textbf{0.23}  & \textbf{0.89}   \\
%\hline
%GloVe + CNN +  Adversarial Training (Demographic Parity) &  1.81 & 1.23  & 0.303 & 0.534 & 0.89 \\
IBP + Adversarial Training & \textbf{0.92}  & 0.358 & \textbf{0.068}  &  0.29  & \textbf{0.901}   \\

\bottomrule
\end{tabular}
\caption{\label{font-table} Experiment results on CNN with GloVe baseline model for Jigsaw dataset. The bolded numbers represent numbers that are statistically significant in difference with the baseline number (p $<$ 0.05). We can see that adding IBP improves fairness. }
\label{table:jigsawresults}
\end{table*}


\begin{table*}[h!]
\centering \small
\begin{tabular}{p{4.5cm}p{2cm}p{1.5cm}p{1.5cm}p{1.5cm}p{2cm}}
\toprule 
\multirow{2}{*}{Model} & {Raw task} & \multicolumn{13}{c}{{Fairness}} & {Robustness}  \\
\cmidrule(lr){2-2}\cmidrule(lr){3-35} \cmidrule(lr){4-46-6}
  &  {AUC}&  {EOdds} & {FPED} & {TPED} & {CRA} \\ 
  \midrule
Baseline  & 0.787 &0.254 & 0.123 &  0.131  & 0.115   \\
  \midrule
IBP &  \textbf{0.743} & 0.26 
& 0.133 & 0.127  & \textbf{0.702}  \\
 IBP_{gender}  &\textbf{0.749} & 0.223  & 0.119 & \textbf{0.104} & \textbf{0.711}    \\
  
 \midrule

Instance weighting & \textbf{0.755} & 0.224  & 0.106 & \textbf{0.118} &  \textbf{0.095}   \\

\textit{HardDebias} &  0.767 &   0.224 & 0.118 &  \textbf{0.106}  & \textbf{0.07}   \\

Adversarial Training  &  0.773 &  0.231  & 0.117 & \textbf{0.114} & \textbf{0.18}   \\
\midrule

IBP + Instance weighting & \textbf{0.732}  &  0.222 &  \textbf{0.109} & \textbf{0.113}   & \textbf{0.719}  \\

IBP + \textit{HardDebias} &  \textbf{0.735} & 0.216 & \textbf{0.115} & \textbf{0.101}  &  \textbf{0.715}  \\

 IBP + Adversarial Training & \textbf{0.725} & 0.226 & \textbf{0.114} &  \textbf{0.112}  & \textbf{0.693}   \\
\bottomrule
\end{tabular}
\caption{\label{font-table} Experiment results on CNN models on Bias in Bios dataset.}
\label{table:ibpresults}
\end{table*}

\begin{table*}[]
\centering
\small
\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}| p{2cm}|}
\hline \textbf{Model} &   \textbf{Raw task AUC} & \textbf{$\text{TPR}_\text{diff}$} & \textbf{CRA} \\
\hline
BERT & 0.796 &  0.148 & 0.164   \\
\hline
BERT + SAFER &  0.129  & 0.134 & 0.726  \\
\hline
BERT + SAFER_{gender} &  0.761 &  \textbf{0.097} & 0.733  \\
\hline
\end{tabular}
\caption{\label{font-table} Model performance on BERT and SAFER for Bias in Bios dataset}
\label{table:bibsaferresults}
\end{table*}



\begin{table*}[h!]
\centering \small
\begin{tabular}{p{4.5cm}p{1.5cm}p{1.5cm}p{2cm}}
\toprule 
\multirow{2}{*}{Model} & {Raw task} & \multicolumn{1}{c}{{Fairness}} & {Robustness}  \\
\cmidrule(lr){2-2}\cmidrule(lr){3-3} \cmidrule(lr){4-4}
  &  {AUC}  & { $\text{TPR}_\text{diff}$ } & {CRA} \\ 
  \midrule
Baseline  & 0.787 &  0.131  & 0.115   \\
  \midrule
IBP &  \textbf{0.743} & 0.127  & \textbf{0.702}  \\
 IBP_{gender}  &\textbf{0.749}& \textbf{0.104} & \textbf{0.711}    \\
  
 \midrule

Instance weighting & \textbf{0.755} & \textbf{0.118} &  \textbf{0.095}   \\

\textit{HardDebias} &  0.767  &  \textbf{0.106}  & \textbf{0.07}   \\

Adversarial Training  &  0.773 & \textbf{0.114} & \textbf{0.18}   \\
\midrule

IBP + Instance weighting & \textbf{0.732}  &   \textbf{0.113}   & \textbf{0.719}  \\

IBP + \textit{HardDebias} &  \textbf{0.735} & \textbf{0.101}  &  \textbf{0.715}  \\

 IBP + Adversarial Training & \textbf{0.725} &  \textbf{0.112}  & \textbf{0.693}   \\
\bottomrule
\end{tabular}
\caption{\label{font-table} Experiment results on CNN models on Bias in Bios dataset.}
\label{table:ibpresults}
\end{table*}


In the baseline CNN model, 37 gender tokens appear in the top-5 features for the baseline model across 34 examples, while only 23 appear in the top-5 features for the IBP model across 21 examples. Similarly for our BERT architecture, 50 gender tokens appeared in the top-5 features of the baseline model across 46 examples, while only 30 appeared in that of the SAFER-trained model across 27 examples. We did not observe any sexual orientation or non-binary gender terms in the top-5 features for either of the models.

There are 133 examples containing at least one gender token among the top 50 features for the baseline model, while there are only 81 examples after training with IBP. This suggests that gender tokens are de-prioritized in the decision making after adding robustness methods. This shows that certified robustness methods helps models be more invariant to spurious gender features.

